The Convergence Rate of SGD's Final Iterate: Analysis on Dimension Dependence

Stochastic Gradient Descent (SGD) is among the simplest and most popular methods in optimization. The convergence rate for SGD has been extensively studied and tight analyses have been established for the running average scheme, but the sub-optimality of the final iterate is still not well-understood. shamir2013stochastic gave the best known upper bound for the final iterate of SGD minimizing non-smooth convex functions, which is $O(\log T/\sqrt{T})$ for Lipschitz convex functions and $O(\log T/ T)$ with additional assumption on strongly convexity. The best known lower bounds, however, are worse than the upper bounds by a factor of $\log T$. harvey2019tight gave matching lower bounds but their construction requires dimension $d= T$. It was then asked by koren2020open how to characterize the final-iterate convergence of SGD in the constant dimension setting. In this paper, we answer this question in the more general setting for any $d\leq T$, proving $\Omega(\log d/\sqrt{T})$ and $\Omega(\log d/T)$ lower bounds for the sub-optimality of the final iterate of SGD in minimizing non-smooth Lipschitz convex and strongly convex functions respectively with standard step size schedules. Our results provide the first general dimension dependent lower bound on the convergence of SGD's final iterate, partially resolving a COLT open question raised by koren2020open. We also present further evidence to show the correct rate in one dimension should be $\Theta(1/\sqrt{T})$, such as a proof of a tight $O(1/\sqrt{T})$ upper bound for one-dimensional special cases in settings more general than koren2020open.

==> scfs.tex <==
\section{Strongly convex functions with $1/\sqrt{T}$ step sizes}
In this section we prove that the final iterate of SGD for non-smooth strongly convex functions has error $\Omega(\log d/ T)$, even in the non-stochastic case. The setting and approach is similar to those in the previous section except that we use a fixed $\eta_t=1/\sqrt{T}$ step size schedule instead.

\begin{theorem}[Main result]
For any $T$ and $1\le d<T$, there exists a convex function $f: X\to \R$ where $X\subset \R^d$, and $f$ is 3-lipschitz and 1-strongly convex. When executing algorithm \ref{alg1} on $f$ with initial point 0 and step size schedule $\eta_t=1/\sqrt{T}$, the last iterate satisfies:
\begin{equation}
    f(x_{T+1})-\min_{x\in X} f(x)\ge \frac{\log d}{5T}
\end{equation}
\end{theorem}

\begin{proof}
Define $f:X \to \R$ and $h_i\in \R^d$ for $i\in[d+1] \cup \{0\}$ by
\begin{align*}
    f(x)=\max_{0\leq i\leq d}H_i(x)
\end{align*}
where $H_i(x)=h_i^\top x+\frac{1}{2}\|x\|^2$. For $i\ge 1$ we define
\begin{align*}
    h_{i, j}=\left\{\begin{array}{ll}
a_{j} & (\text { if } 1 \leq j<i) \\
-1 & (\text { if } i=j \leq d) \\
0 & (\text { if } i<j \leq d)
\end{array} \quad \text { and } \quad a_{j}=\frac{1}{2(d+1-j)} \quad(\text { for } j \in[d] )\right.
\end{align*}

Additionally, let $h_0=0$ and $H_0(x)=\frac{1}{2}\|x\|^2$. It's easy to check that $f$ is 3-lipschitz and 1-strongly convex, with a non-positive minimal value. We have the following standard claim.

\begin{claim}
$\partial f(x)$ is the convex hull of $\{h_i+x\mid i\in {\cal I}(x)\}$ where ${\cal I}(x)=\{i\geq 0\mid H_i(x)=f(x)\}$.
\end{claim}

Our non-stochastic sub-gradient oracle outputs 0 for the first $T-d$ steps and outputs $h_{i'}+x$ where $i'=\min{\cal I}(x) \setminus \{0\}$ for the last $d$ steps. Define $z_1=\cdots =z_{T-d+1}=0$, let $T-d=T^*$ 
\begin{align*}
    z_{t,j}=\left\{\begin{array}{ll}
       \frac{1-(t-T^*-j-1)a_j}{\sqrt{T}}  & (\text{ if } 1\leq j<t-T^*)  \\ 
        0 & (\text{ if } t-T^* \leq j \leq T)
    \end{array} \right. \quad (\text{ for } t>T^*+1).
\end{align*}

We will show inductively that these are precisely the first $T$ iterates produced by algorithm \ref{alg1} when using the sub-gradient oracle defined above. The following claim is obvious from definition.

\begin{claim}
We have the following claims:
\begin{itemize}
    \item $z_t$ is non-negative. In particular, $z_{t,j}\geq \frac{1}{2(t-1)}$ for $j<t-T^*$ and $z_{t,j}=0$ for $j\geq t-T^*$.
    \item $z_t=0$ for $t\in [T^*]$ and $\|z_t\|^2\leq \frac{1}{t-1}$ for $t>T^*+1$. Thus $z_t\in X$.
\end{itemize}
\end{claim}

We can now determine the value and sub-differential at $z_t$. The case for the first $T^*$ steps is trivial as the sub-gradient oracle always outputs 0 and $x_1$ never moves a bit. For the last $d$ steps we have the following claim.
\begin{claim}
$f(z_t)=H_{t-T^*}(z_t)$ for all $T^*<t\leq T+1$. The subgradient oracle for $f$ at $z_t$ returns the vector $h_t+z_t$.
\end{claim}

\begin{proof}
We claim that $h_{t-T^*}^\top z_t=h_{i-T^*}^\top z_t$ for all $i>t>T^*$. 
By definition, $z_t$ is supported on its first $t-T^*$ coordinates, completing the first part of the claim. Next we claim that $z_t^\top h_{t-T^*}> z_t^\top h_{i-T^*}$ for all $T^*+1\leq i <t$. For $T^*\leq i<t$, one has
\begin{align*}
    z_t^\top (h_{t-T^*}-h_{i-T^*})=\sum_{j=i}^{t-1}z_{t,j}(h_{t-T^*,j}-h_{i-T^*,j})=z_{t,i}(a_i+1)+\sum_{j=i+1}^{t-1}z_{t,j}a_j>0.
\end{align*}

The two claims guarantee that $f(z_t)=H_{t-T^*}(z_t)$. Combining with the fact ${\cal I}(z_t)=\{t,...,T+1\}$, we conclude that the sub-gradient oracle outputs $h_{t-T^*}+z_t$.
\end{proof}

From the above claim we have that the vector $x_t$ in algorithm \ref{alg1} is equal to $z_t$ for $t\in [T+1]$, which allows determination of the value of the final iterate:
\begin{align*}
    f(x_{T+1})=f(z_{T+1})=H_{d+1}(z_{T+1})\geq \sum_{j=1}^{d+1}h_{d+1,j}z_{T+1,j}\geq \sum_{j=1}^{d+1} \frac{1}{2(d+1-j)}\frac{1}{2T}>\frac{\log d}{5T}.
\end{align*}
\end{proof}

==> sgd_onedim.tex <==
\section{SGD in one-dimension}

\begin{theorem}[Freedman's Inequality, Theorem 1.6 in~\cite{Fre75}]
\label{thm:FreedmanInequality}
Consider a real-valued martingale sequence $\{X_t\}_{t\geq 0}$ such that $X_0=0$, and $\E[X_{t+1}|\mathcal{F}_t]=0$ for all $t$, where $\{\mathcal{F}_t\}_{t\geq 0}$ is the filtration defined by the martingale. Assume that the sequence is uniformly bounded, i.e., $|X_t|\leq M$ almost surely for all $t$. Now define the predictable quadratic variation process of the martingale to be $W_t=\sum_{j=1}^t \E[X_j^2|\mathcal{F}_{j-1}]$ for all $t\geq 1$. Then for all $\ell \geq 0$ and $\sigma^2>0$ and any stopping time $\tau$, we have
\[
\Pr\Big[ \Big|\sum_{j=0}^\tau X_j \Big|\geq \ell \wedge W_\tau \leq \sigma^2 \text{for some stopping time } \tau \Big] \leq 2\exp\Big(- \frac{\ell^2/2}{\sigma^2+M \ell/3} \Big).
\]
\end{theorem}



\begin{definition}
We define a set of good points by $\Scal$, which contains all ideal points:
\begin{align*}
    \Scal=\{x\in \K:f(x)-f^*\leq \frac{GD}{\sqrt{T}}\}.
\end{align*}
\end{definition}

\begin{lemma}
For any $x\in \K\setminus\Scal$, one has
\begin{align*}
    |\nabla f(x)|>\frac{G}{\sqrt{T}}.
\end{align*}
\end{lemma}

\begin{proof}
We prove this statement by contradiction. 
Suppose $x\in\K\setminus \Scal$ subject to $|\nabla f(x)|\leq \frac{G}{\sqrt{T}}$. 
By the convexity of $f$ and the definition of sub-gradient and let $x^*\in \K$ be a minimizer (arbitrarily if the minimizers are not unique), one has
\begin{align*}
    f(x^*)\geq f(x)+ \nabla f(x) (x-x^*),
\end{align*}
which implies that
\begin{align*}
    f(x)-f(x^*)\leq & \nabla f(x) (x^*-x)\leq \frac{GD}{\sqrt{T}}.
\end{align*}
Contradiction.
\end{proof}

Let $s_L=\inf_{x\in\Scal}x$ and $s_R=\sup_{x\in\Scal}x$.
\begin{definition}
We define the distance from a point the set of good points as follows:
\begin{align*}
    \|x-\Scal\|=\left\{\begin{array}{ll}
n_{L}-x & \text { if } x<n_{L} \\
0 & \text { if } \quad n_{L} \leq x \leq n_{R} \\
x-n_{R} & \text { if } x>n_{R}
\end{array}\right.
\end{align*}
\end{definition}
Suppose we start from an arbitrary point $x_0\in \K$ and the (random) sequence is denoted by $x_0,x_1,\cdots,x_T$.


\begin{lemma}
We are given any $x_0\in \K$.
Let $\tau=:\min_{i}\{1\leq i\leq t+1\mid x_{i}\in \Scal\}$  and $\tau:=\infty$ if SGD never goes back to the set of good points in the first $t$ steps.
If $t\geq T/2$, we know that
\begin{align*}
    \Pr[\tau=\infty\mid x_0]\leq 2\exp{-\Omega(\sqrt{T})}.
\end{align*}
\end{lemma}

\begin{proof}
Without loss of generality, we consider the case when $x_i> n_R$ for all $1\leq i\leq t$ and we do not do projection in the SGD.
As doing projection only decreases the objective probability.

We define a random variable $y_i=x_i-x_{i-1}$ to capture the movement of the solution for $1\leq i\leq t+1$.
Conditioning on $\tau =\infty$, i.e. $x_i>n_R$ for all $1\leq i\leq t+1$, we know that $\E[y_i]\leq -\eta \frac{G}{\sqrt{T}}=-4D/T$ for $i\geq 2$.
Let $\F_i$ be the filtration and $\Tilde{y}_i=y_i-\E[y_i\mid \F_i]$.
It is easy to verify that $\{\Tilde{y}_{i}\}$ is a martingale:
\begin{align*}
    \E[\Tilde{y}_i\mid \F_{i}]=\E[y_i\mid \F_i]-\E[y_i\mid\F_i]=0.
\end{align*}

Obviously, one has $|\Tilde{y}_i|\leq \frac{4D}{G\sqrt{T}}$.
Let $\ell=|\sum_{i=1}^{t}\E[y_i]|.$ We know that $W_t=\sum_{i=1}^t \E[\Tilde{y_i}^2\mid \F_{i-1} ]\leq \eta G| \sum_{i=1}^t \E[y_i\mid \F_{i-1}]|$.
We have
\begin{align*}
    \Pr[\tau=\infty\mid x_0]\leq & \Pr[\sum_{i=1}^{t}y_i\geq -D]\\
    \leq & \Pr[|\sum_{i=1}^t \Tilde{y_i}|\geq \ell-D\wedge W_t\leq \eta G\ell]\\
    \leq & 2\exp\big(-\frac{(\ell-D)^2}{\eta Gl+\frac{4D}{3G\sqrt{T}}\ell}\big).
\end{align*}
If $t\geq T/2$, we know that $\ell\geq 2D$ and the statement follows directly by elementary calculation.
\end{proof}

\begin{lemma}
One has
\begin{align*}
    \E[ \|x_t-\Scal\|\mid \tau=\infty\wedge x_0]\leq O(\frac{GD}{\sqrt{T}}).
\end{align*}
\end{lemma}
\begin{proof}
The proof is similar to the previous one by constructing martingale and using the Freedman's Inequality.

\begin{align*}
    \Pr[\|x_t-\Scal\|>k, \tau =\infty\mid x_0]=\Pr[\tau=\infty\mid x_0]\cdot \Pr[\|x_t-\Scal\|>k\mid \tau=\infty,x_0]
\end{align*}

We have 
\begin{align*}
    \Pr[\|x_t-\Scal\|> k, \tau=\infty \mid x_0]
\end{align*}
\end{proof}

\begin{lemma}
For any $x_0\in \Scal$, we know that
\begin{align*}
    \E[\|x_T-\Scal\| \mid x_0]\leq \frac{2D}{\sqrt{T}}.
\end{align*}
\end{lemma}
\begin{proof}

We prove this by induction.
For the base case, one has
\begin{align*}
    \E[\|x_1-\Scal \|\mid x_0]\leq \E[\|x_1-x_0|+\|x_0-\Scal\|\mid x_0]\leq \frac{D}{\sqrt{T}}.
\end{align*}

Assume this statement holds for all $t'\in [1,t-1]$, and we want to bound $\E[ \|x_t-\Scal \|\mid x_0]$. 
We define a random variable $\tau$ in the inductive step to indicate the first positive time at which the SGD algorithm gets a good point.
More specifically, $\tau=:\min_{t'}\{1\leq t'\leq t\mid x_t\in \Scal\}$  and $\tau:=\infty$ if SGD never goes back to the set of good points in the first $t$ steps.
\begin{align*}
    \E[\|x_t-\Scal\|\mid x_0]=& \sum_{k=1}^{t}\Pr[\tau=k\mid x_0]\E[\|x_t-\Scal\|\mid \tau=k\wedge x_0]+\Pr[\tau=\infty\mid x_0]\E[ \|x_t-\Scal\|\mid \tau=\infty\wedge x_0].
\end{align*}

By the inductive hypothesis, we know that $\E[\|x_t-\Scal\|\mid \tau=k\wedge x_0 ] \leq \frac{2D}{\sqrt{T}}$.
It suffices to prove that

\end{proof}


